Personalized Top-k Set Queries Over Predicted Scores

This work studies the applicability of expensive external oracles such as large language models in answering top-k queries over predicted scores. Such scores are incurred by user-defined functions to answer personalized queries over multi-modal data. We propose a generic computational framework that handles arbitrary set-based scoring functions, as long as the functions could be decomposed into constructs, each of which sent to an oracle (in our case an LLM) to predict partial scores. At a given point in time, the framework assumes a set of responses and their partial predicted scores, and it maintains a collection of possible sets that are likely to be the true top-k. Since calling oracles is costly, our framework judiciously identifies the next construct, i.e., the next best question to ask the oracle so as to maximize the likelihood of identifying the true top-k. We present a principled probabilistic model that quantifies that likelihood. We study efficiency opportunities in designing algorithms. We run an evaluation with three large scale datasets, scoring functions, and baselines. Experiments indicate the efficacy of our framework, as it achieves an order of magnitude improvement over baselines in requiring LLM calls while ensuring result accuracy. Scalability experiments further indicate that our framework could be used in large-scale applications.

==> abstract_old.tex <==
\begin{abstract}
This work studies the applicability of expensive external oracles (e.g., deep neural networks, large language models) in answering top-$k$ queries over predicted scores. Such scores are incurred by user defined scoring functions over multi-modal data. We propose a generic computational framework that handles arbitrary set based scoring functions, as long as the  functions could be decomposed into constructs, each of which could be sent to an oracle to predict partial scores. At a given point in time, the framework assumes a set of responses and their partial predicted scores, and it maintains a set of possible sets that are likely to be the true top-$k$. Since calling oracles is costly, our framework judiciously identifies the next construct, i.e., the next best question, to be asked to the oracle such that the response to this question has the maximum likelihood of identifying the true top-$k$. We model an oracle's response to be deterministic or probabilistic and propose a principled probabilistic model that quantifies the likelihood of a candidate set to be the true top-$k$ to identify the next best question. We study a suite of efficiency opportunities in designing different tasks in our framework. We run an evaluation with multiple datasets, scoring functions, and  appropriate baselines. Our experimental results corroborate our theoretical analysis.
\end{abstract}

==> algorithms_old.tex <==
\section{Algorithms for the framework}
\label{section3}

\subsection{Identifying the Candidates' Set}
\label{candidatesset}

\begin{definition}
    \textbf{Candidates Set}: The set of candidates which have a chance to be the query answer.
\end{definition}
 To identify the candidates set, we must ensure it includes any potential query answer while excluding any candidates that can be definitively ruled out as the query answer.
 Ultimately, our goal is to choose a candidate among all which has the highest score in the candidates set with respect to the scoring function. In other words:

\[
\text{Query answer = } \arg\max_{c \in \text{C}} \mathcal{F}(c, q)
\]
Where \(\text{C}\) is the candidates set.

\begin{example}
    Given $n$ entities and a fixed $k$, there are \( \binom{n}{k} \) unique combinations of k entities. Depending on the scoring function and the context of the problem, a subset or the whole set of such candidates form the candidates set. Considering the running example to find out the top-3 hotels among the 5 ones mentioned in \autoref{tab:ny_hotels_relevance}, there can be \( \binom{5}{3} = 10 \) sets of size 3 among the whole 5 hotels. Hence, assuming all possible combinations have a chance to be the top-3 set, we will have:
    \[
    \text{C} = 
    \begin{cases}
    c_1 = \{ \text{HNY}, \text{MLN}, \text{HYN} \}, & c_2 = \{ \text{HNY}, \text{MLN}, \text{SHN} \} \\
    c_3 = \{ \text{HNY}, \text{MLN}, \text{WLD} \}, & c_4 = \{ \text{HNY}, \text{HYN}, \text{SHN} \} \\
    c_5 = \{ \text{HNY}, \text{HYN}, \text{WLD} \}, & c_6 = \{ \text{HNY}, \text{SHN}, \text{WLD} \} \\
    c_7 = \{ \text{MLN}, \text{HYN}, \text{SHN} \}, & c_8 = \{ \text{MLN}, \text{HYN}, \text{WLD} \} \\
    c_9 = \{ \text{MLN}, \text{SHN}, \text{WLD} \}, & c_{10} = \{ \text{HYN}, \text{SHN}, \text{WLD} \} 
    \end{cases}
\]

Initially, we may exclude a subset of these candidates that are assuredly not the query answer, based on prior knowledge on the context of the problem. 

\end{example}


%Example: hotels with initial score, first update on bounds

%Now, assume another table of already called and obtained bounds, consider two questions which one results in finding the winner? hence, we pick question that reduces the ucertainty the most. but how to measure uncertainty of a candidate set?

\subsection{Bounds Computation of Candidates' Set}
\label{bound_computation}

After having the candidates specified, Our goal is to find out the one which has the highest score among all. Since we do not know the exact scores for the candidates, we model the score of a candidate as a tuple of Lower Bound (LB) and Upper Bound (UB) score such that we ensure the candidate's score is within that bound. 

\begin{definition}
    \textbf{Candidate Bounds}: Given a scoring function $\mathcal{F}(c, q)$ and known information $Q_k$, the bounds $(LB_c, UB_c)$ for candidate c are the minimum and maximum overall score of $c$ with respect to $Q_k$. Hence, we have:
    \[
    LB_c \leq \mathcal{F}(c, q) \leq UB_c
    \]
\end{definition}


Where (LB\_c, UB\_c) is calculated based on $\mathcal{F}(c, q)$ and $Q_k$. These bounds need to be kept updated when new information (response to a question) is appended to $Q_k$. 

\begin{comment}

\begin{definition}[Candidates Set Bounds]
\label{candidate_set} Given a scoring function $\mathcal{F}$ and n candidates, candidates set Bounds represent the score bounds for each candidate at a point in time. candidates set Bounds (C) can be represented as follows:

\[
\text{C} = \{ c_1:(\text{LB}_{c_1}, \text{UB}_{c_1}), c_2: (\text{LB}_{c_2}, \text{UB}_{c_2}), \ldots, c_n:(\text{LB}_{c_n}, \text{UB}_{c_n}) \}
\] 
\end{definition}

After each question from the LLM, the bounds for the candidates need to be updated. 
\end{comment}
Algorithm 1 represents the procedure for updating the bounds of the candidates set after a question $Q$ is asked from expert. Depending on what components the scoring function \( \mathcal{F}(c, q) \) is composed of, different types of questions may contribute to the overall score of a candidate, and how these questions contribute to the overall score depends on the exact formula of \( \mathcal{F}(c, q) \). Let \( Q_c \) represent the set of all questions that contribute to the total score of candidate \( c \). If $Q \in Q_c$, then the bounds of $c$ needs to be updated since $Q$ is not unknown anymore. 

\begin{algorithm}
\caption{Update Bounds for Candidates}
\begin{algorithmic}[1]
\State \( res \leftarrow LLM(Q) \)
\For{each candidate \( c \in C \)}
    \State \( Q_c \leftarrow \) set of all questions contributing to the score of \( c \)
    \If{\( Q \in Q_c \)}
        \State Substitute \( Q \) with \( res \) in the formula of \( \mathcal{F}(c, q) \)
        \State \( LB_c \gets \min_{Q_u} \mathcal{F}(c, q) \)
        \State \( UB_c \gets \max_{Q_u} \mathcal{F}(c, q) \)
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{comment}
   \begin{algorithm}
\caption{Update Bounds for Candidates}
\begin{algorithmic}[1]
\State \( res \leftarrow LLM(Q) \)
\For{each candidate \( c \in C \)}
    \State \( Q_c \leftarrow \) set of all questions contributing to the score of c
    \If{\( Q \in Q_c \)} 
        \If{scoring function is based on sum}
            \State \( LB_c \gets LB_c + res \) 
            \State \( UB_c \gets UB_c - (MAX\_SCORE - res) \)
        \ElsIf{scoring function is based on average}
            \State \( n \gets \text{len}(Q_c) \)
            \State \( LB_c \gets LB_c + \frac{res}{n} \) 
            \State \( UB_c \gets UB_c - \frac{MAX\_SCORE - res}{n} \)
        \EndIf
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm} 
\end{comment}


\begin{example}
Given the running example with $\mathcal{F}_{\text{rel+div}}(c, q)$ as the scoring function, let's consider the starting point in time, when no had been inserted in \autoref{tab:ny_hotels_relevance} and \autoref{tab:ny_hotels_diversity}. In this case:
\[
Q_k = \emptyset
\]

To establish the initial bounds for all candidates, we define the minimum and maximum possible scores based on the scoring formula \(\mathcal{F}_{\text{rel+div}}(c, q)\). Given that \(k = 3\), for an arbitrary candidate \(c = \{e_1, e_2, e_3\}\), we express the score as follows:

\begin{align*}
\mathcal{F}(c, q) &= \sum_{e \in c} \text{Rel}(q, e) + \sum_{e_i, e_j \in c} \text{Div}(e_i, e_j) \\
&= \text{Rel}(q, e_1) + \text{Rel}(q, e_2) + \text{Rel}(q, e_3) \\
&\quad + \text{Div}(e_1, e_2) + \text{Div}(e_1, e_3) + \text{Div}(e_2, e_3)
\end{align*}

It is specified that each score obtained as the expert response for any \(\text{Rel}\) or \(\text{Div}\) question lies within the range \((0, 1)\). On the other hand, as shown in the above formula, there are 6 questions contributing to the overall score of an arbitrary candidate. Therefore, initially, the lower and upper score bounds for all candidates are defined as follows:

\begin{align*}
\text{LB}(c_i) &= \text{MIN\_SCORE} = 0 \quad \forall c_i \in \text{candidates} \\
\text{UB}(c_i) &= \text{MAX\_SCORE} = 6 \quad \forall c_i \in \text{candidates}
\end{align*}

Hence, We can represent the initial candidates set with their corresponding bounds as follows:

\[
    \text{C} = 
    \begin{cases}
    c_1 = \{ \text{HNY}, \text{MLN}, \text{HYN} \}, & c_2 = \{ \text{HNY}, \text{MLN}, \text{SHN} \} \\
    c_3 = \{ \text{HNY}, \text{MLN}, \text{WLD} \}, & c_4 = \{ \text{HNY}, \text{HYN}, \text{SHN} \} \\
    c_5 = \{ \text{HNY}, \text{HYN}, \text{WLD} \}, & c_6 = \{ \text{HNY}, \text{SHN}, \text{WLD} \} \\
    c_7 = \{ \text{MLN}, \text{HYN}, \text{SHN} \}, & c_8 = \{ \text{MLN}, \text{HYN}, \text{WLD} \} \\
    c_9 = \{ \text{MLN}, \text{SHN}, \text{WLD} \}, & c_{10} = \{ \text{HYN}, \text{SHN}, \text{WLD} \} 
    \end{cases}
\]

\[
\text{C\_bounds} = \{ c_1: (0, 6), c_2: (0, 6), c_3: (0, 6), \ldots, c_{10}: (0, 6) \}
\]

Let's say we decide to ask \( R(WLD, q) \) first, and the LLM returns \( R(WLD, q) = 0.5 \). Hence, we need to update the lower bound (LB) and upper bound (UB) scores of those candidates containing \( WLD \). These candidates are \( c_3 \), \( c_5 \), \( c_6 \), \( c_8 \), \( c_9 \), and \( c_{10} \). As an example, for \( c_3 \), we will have:
\begin{align*}
\mathcal{F}(c_3, q) & = R(HNY, q) + R(MLN, q) + R(WLD, q) + D(HNY, MLN) \\
          & \quad + D(HNY, WLD) + D(MLN, WLD) \\
          & = R(HNY, q) + R(MLN, q) + 0.5 + D(HNY, MLN) \\
          & \quad + D(HNY, WLD) + D(MLN, WLD) \\
          & \implies 0.5 \leq \mathcal{F}(c_3, q) \leq 5.5
\end{align*}

Similarly, we update the bounds for \( c_{5} \), \( c_{6} \), \( c_{8} \), \( c_{9} \), and \( c_{10} \). The new candidate set bounds are as follows:

\[
\text{candidates\_set\_bounds} = \{ 
\begin{aligned}
c_1 &: (0, 6), & c_2 &: (0, 6), \\
c_3 &: (0.5, 5.5), & c_4 &: (0, 6), \\
c_5 &: (0.5, 5.5), & c_6 &: (0.5, 5.5), \\
c_7 &: (0, 6), & c_8 &: (0.5, 5.5), \\
c_9 &: (0.5, 5.5), & c_{10} &: (0.5, 5.5) 
\end{aligned}
\}
\]


This candidates set corresponds to a specific time \( t = 1 \), which only \( R(WLD, q) \) has been asked. When the next question is asked (\( t = 2 \)), the candidates set will be updated again.

Now, at (\( t = 2 \)), let's assume we choose a diversity question like \( D(HNY, MLN) \) to ask. \autoref{tab:ny_hotels_diversity} represents the diversity scores for each pair of hotels. Hence, the expert response is \(1.0\) as \( D(HNY, MLN) = 1.0\) in this table. Now, we need to update candidates including both HNY and MLN, which are \( c_{1} \), \( c_{2} \), and \( c_{3} \). For instance, for \( c_{3} \) we will have:

\begin{align*}
\mathcal{F}(c_3, q) & = R(HNY, q) + R(MLN, q) + 0.5 + D(HNY, MLN) \\
          & \quad + D(HNY, WLD) + D(MLN, WLD) \\
          & = R(HNY, q) + R(MLN, q) + 0.5 + 1.0 \\
          & \quad + D(HNY, WLD) + D(MLN, WLD) \\
          & \implies 1.5 \leq \mathcal{F}(c_3, q) \leq 5.5
\end{align*}

Similarly, we update the bounds for \( c_{1} \) and \( c_{2} \). The new candidates set bounds are as follows:

\[
\text{candidates\_set\_bounds} = \{ 
\begin{aligned}
c_1 &: (1.0, 6), & c_2 &: (1.0, 6), \\
c_3 &: (1.5, 5.5), & c_4 &: (0.0, 6.0), \\
c_5 &: (0.5, 5.5), & c_6 &: (0.5, 5.5), \\
c_7 &: (0.0, 6.0), & c_8 &: (0.5, 5.5), \\
c_9 &: (0.5, 5.5), & c_{10} &: (0.5, 5.5)
\end{aligned}
\}
\]

Finally, let's assume we are at the current point in time, when we have asked all the questions which have known values in \autoref{tab:ny_hotels_relevance} and \autoref{tab:ny_hotels_diversity}, resulting in those two tables. If we update the bounds accordingly based on all the known values, we will have up-to-date bounds as follows:

\[
\text{candidates\_set\_bounds} = \{ 
\begin{aligned}
c_1 &: (3.5, 5.5), & c_2 &: (2.5, 4.5), \\
c_3 &: (3.0, 5.0), & c_4 &: (2.0, 4.0), \\
c_5 &: (3.0, 4.0), & c_6 &: (1.5, 3.5), \\
c_7 &: (2.0, 5.0), & c_8 &: (3.0, 5.0), \\
c_9 &: (1.5, 4.5), & c_{10} &: (2.0, 4.0)
\end{aligned}
\}
\]

\end{example}


\subsection{Probabilistic Model for finding the winner}
\label{winning_probability}

In \autoref{bound_computation} we showed how to maintain and update the score bounds for each candidate after we get new information (response to a question) from an expert. We need to keep asking questions from expert and update bounds accordingly as long as the query answer is not determined, and the query answer is the candidate which we ensure has the highest score compared to others. We refer to such a candidate as the winner candidate and define it as follows:

\begin{definition}[Winner Candidate]
A candidate \( c^* \) is referred to as the \textit{Winner Candidate} if its lower bound is greater than or equal to the upper bounds of all other candidates. Mathematically, this condition can be expressed as:

\[
\text{LB}(c^*) \geq \text{UB}(c_i) \quad \forall c_i \in \text{C}, \
\]

\end{definition}

Our ultimate goal is to find $c^*$, and if $c^*$ is unknown at a point in time, meaning that there is no candidate that satisfies the above constraint, it indicates uncertainty in determining the winner, and more questions must be asked from the expert to update the bounds again and reduce uncertainty. We will formally define uncertainty of a candidates set in \autoref{uncertainty}.

In order to find the winner candidate, in this subsection, we formalize the probability distribution function of the winner candidate c*. In other words, we demonstrate how to compute the probability of any arbitrary candidate to be the winner at a given point in time. In \autoref{uncertainty}, we use this probability distribution function (PDF) to demonstrate what is the best next question to ask expert which maximally reduces the uncertainty of finding the winner candidate. Ultimately, we look for a time step in which $c^*$ is known, which means zero uncertainty in finding the winner candidate. 

\textbf{Question:} Given a candidates set $C$ with corresponding bounds for each candidate, and a specific candidate $c \in C$, what is the probability that $c = c^*$?

\begin{comment}
In order to find this probability, we consider two different cases. 

\textbf{Case 1 - Independence assumption}: In this case, we assume that the candidates are independent. Hence, we can compute $P(c = c^*)$ as follows:

% example

\[
P(c = c^*) = \prod_{c' \in C} P(\mathcal{F}(c, q) \geq \mathcal{F}(c', q))
\]

\textbf{\textcolor{red}{An example needs to be added here}}

\end{comment}
Generally, Candidates can potentially be dependent since they have common entities among them. Hence, we do not consider the Independence assumption between candidates, and compute the exact probabilities with no prior assumption. Hence, we can formalize $P(c = c^*)$ as follows:

\begin{align*}
P(c = c^*) &= P\left(\bigwedge_{c' \in C} \mathcal{F}(c, q) \geq \mathcal{F}(c', q)\right)
\end{align*}



This can be expanded as the product of conditional probabilities:

\[
P(c = c^*) = \prod_{i=1}^{n} P\left(\mathcal{F}(c, q) \geq \mathcal{F}(c_i, q) \mid \bigcap_{j=1}^{i-1} \left( \mathcal{F}(c, q) \geq \mathcal{F}(c_j, q) \right) \right)
\]

This formula is basically a multiplication of probabilities of the following type:

\[
P(\mathcal{F}(c, q) \geq \mathcal{F}(c_i, q) \mid \bigcap_{j=1}^{i-1} \left( \mathcal{F}(c, q) \geq \mathcal{F}(c_j, q) \right))
\]

Hence, We need to compute probabilities of the following the form:

\[
P(f(c_1) \geq f(c_2) \mid \text{constraints})
\]

This probability represents the likelihood that candidate \( c_1 \) scores higher than candidate \( c_2 \), given a set of constraints imposed by previous comparisons between candidates.

To compute this probability, we can rewrite it as follows:

\[
P(f(c_1) > f(c_2) \mid \text{constraints}) = \frac{p((f(c_1) \geq f(c_2)) \land \text{constraints})}{p(\text{constraints})} 
\]
\[
= \frac{n((f(c_1) \geq f(c_2)) \land \text{constraints})}{n(\text{constraints})}
\]

Where the denominator represents the size or number of all possible score assignments to candidates that satisfy the given constraints. Similarly, The numerator is just the size of a subset of  scoring assignments of the denominator that capture the additional constraint: \( f(c_1) \geq f(c_2) \). 

There are two key points that we address to compute the probabilities efficiently and accurately:

\begin{enumerate}
    \item \textbf{Storage bottleneck.} Generally, given n candidates, we can use a n-dimensional table to represent all the possible combinations of score assignment for the $n$ candidates. Then, among cells of this table that satisfy the constraints, we can compute what proportion of them satisfy the additional constraint (\( f(c_1) > f(c_2) \)) as well, and this proportion gives us the desired probability. However, let's say each candidate has m different score values. Then, the n-dimensional table has space complexity of $O(m^n)$. Therefore, it requires a huge amount of memory to compute probabilities with this approach. Basically, many of the cells in this n-dimensional table are unnecessary to store. To overcome the storage bottleneck for computing $P(c = c^*$), we do not store any n-dimensional tables. 
    
    $P(c = c^*$) is basically computing a sequence of pairwise probabilities between candidates given a set of constraints for each probability.  Hence, instead of sotring a n-dimensional table, we just consider a vector of possible score values for the first two candidates in the sequence of probabilities that we want to compute, and do cartesian product between them and compute what ratio of the combination of their values satisfies the constraints. In this say, the result of the first term in the probability sequence is obtained. Then, we do the next cartesian prodoct between the result from the previous step and the corresponding vector of the next candidate in the sequence. We repeat the same procedure until we have computed all the terms in the probability sequence of $P(c = c^*$). Then, we can get the final result by multiplying the results obtained from each step. In this approach, we only need to store the result obtained from the most recent step in probability calculation. Hence, the space complexity of computing probabilities is reduced to $O(m)$ where $m$ is the maximum size of a candidate's corresponding vector, or equivalently, number of possible values for score of a candidate. In example 3.6, we will further elaborate on this probability computation.
    \item \textbf{Computing} $\mathbf{f(c_1) \geq f(c_2).}$ Given two candidates $c1$ and $c2$, if the two candidates have common entities in between and we want to compute $P(\mathcal{F}(c, q) \geq \mathcal{F}(c_j, q))$, we cannot just rely on the bounds of $c_1$ and $c_2$ to compute the probability because since they have common entities, they have one or more common unknown questions, and we need to eliminate the effect of common unknown questions between $c1$ and $c2$ to compute the probability. This is bacause if we know a common unknown question between two candidates, it is  going to have the exact same effect on the two candidates. To eliminate the effect of such questions, we may assume that they do not have any effect on the bounds of $c_1$ and $c_2$, and compute the probabilities with this further assumption. 
\end{enumerate}

In example 3.6, we will elaborate how to compute probabilities while addressing the two mentioned key points. 

\begin{example}
    Given the bounds obtained from the example in \autoref{winning_probability}, let's assume there are only the first three candidates, which are as follows:

    \[
    \text{Candidates\_Set\_Bounds} = 
    \left\{ 
    \begin{array}{ll}
    c_1 & : \quad (3.5, 5.5), \\ 
    c_2 & : \quad (2.5, 4.5), \\ 
    c_3 & : \quad (3.0, 5.0)
    \end{array}
    \right\}
\]


    We have already assumed that the processed responses are from the discrete set $S = \{0.0, 0.5, 1.0\}$. Hence, the overall score of any arbitrary candidate should be a multiple of $0.5$ within the range specified by the candidate bounds. 

    In this example, For simplicity of notation, we replace $P(\mathcal{F}(c_i) \geq \mathcal{F}(c_j))$ by $P(c_i \geq c_j)$. Assume we are interested in calculating the probability that \( c_2 \) is the winning candidate (query answer), denoted as \( P(c_1 = c^*) \). This is formulated as:

    \[
    P(c_2 = c^*) = P(c_2 \geq c_1, \, c_2 \geq c_3) = P(c_2 \geq c_1) \cdot P(c_2 \geq c_3 \mid c_2 \geq c_1).
    \]

    To compute each term in this probability sequence, we use the result from the previous term sequentially. Since there are two terms in the above sequence, we break the problem down into two parts as follows: 
    
\textbf{(a)} \(\mathbf{P(c_2 \geq c_1)}\)


To compute this probability, we need to consider the cartesian product $c_1 \times c_2$. Then, \autoref{fig:Example_3_6_a}(a) shows how we only select a subset of all combinations of $c_1$ and $c_2$ which satisfy $c_2 \geq c_1$ by representing these combinations of satisfying values with arrows. For ease of demonstration, we have used different colors for different values of $c_2$.

Since each $c_1$ and $c_2$ have 5 possible values, there are $25$ different combinations between them, and since there are 6 arrows, it means 6 of them satisfy: $c_2 \geq c_1$. Hence, if $c_1$ and $c_2$ had no unknown questions in common (any unknown question that influences both candidates), then, we could conclude that: \(\mathbf{P(c_2 \geq c_1)} = \frac{6}{25}\). However, they have one unknown question in common which is $R(HNY, q)$ and we need to eliminate its effect on the result of this probability. To do this, we assume that $R(HNY, q) = 0$ which means it has no effect on the bounds of $c_1$ and $c_2$ particularly for computing \(\mathbf{P(c_2 \geq c_1)}\). We only do this for computing the final numerical result of a probability term, and keep the original bounds as they are when we want to use them for the next probability term. Hence, assuming $R(HNY, q) = 0$, we have the new bounds as follows:

\[
    \text{Bounds} = 
    \left\{ 
    \begin{array}{ll}
    c_1 & : \quad (3.5, 4.5), \\ 
    c_2 & : \quad (2.5, 3.5)
    \end{array}
    \right\}
\]

These tightened temporary bounds eliminate some of the arrows in \autoref{fig:Example_3_6_a}(a), and change it to \autoref{fig:Example_3_6_a}(b). Hence, after applying the removal of common elements' effect, since there are 9 possible values and there is one arrow, we have:

\(\mathbf{P(c_2 \geq c_1)} = \frac{1}{9}\)


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/Example_3_6_a.jpg}
    \caption{Computing \(\mathbf{P(c_2 \geq c_1)}\)}
    \label{fig:Example_3_6_b}
\end{figure}

\textbf{(b)} \(\mathbf{P(c_2 \geq c_3 \mid c_2 \geq c_1)}\)

\autoref{fig:Example_3_6_b}(a) Shows all the possible values combination of $(c_1, c_2, c_3)$ such that $c_2 \geq c_3$ given $c_2 \geq c_1$ as the assumption. However, just as described before, we need to eliminate the effect of common unknown questions between $c_2$ and $c_3$. $R(HNY, q)$ is the only common unknown question between $c_2$ and $c_3$. Hence, assuming it is zero, we get the temporary bounds of $c-2$ and $c_3$ as follows:

\[
    \text{Bounds} = 
    \left\{ 
    \begin{array}{ll}
    c_2 & : \quad (2.5, 3.5), \\ 
    c_3 & : \quad (3.0, 4.0)
    \end{array}
    \right\}
\]

These tightened temporary bounds eliminate some of the arrows in \autoref{fig:Example_3_6_b}(a), and change it to \autoref{fig:Example_3_6_b}(b). Hence, after applying the removal of common elements' effect, since there are $3 \times 5 \times 3$ possible assignments of values and there are two ingoing arrows to $c_3$, we have:

\(\mathbf{P(c_2 \geq c_3 \mid c_2 \geq c_1)} = \frac{2}{45}\)


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/Example_3_6_b.jpg}
    \caption{Computing \(\mathbf{P(c_2 \geq c_1)}\)}
    \label{fig:Example_3_6_a}
\end{figure}

Finally, we can multiply the obtained  results from part (a) and part(b) to get $P(c_2 = c^*)$. Similarly, the probabilities \( P(c_2 = c^*) \) and \( P(c_3 = c^*) \) can be computed to derive the complete probability distribution of the winning candidate $c^*$ across all possible candidates as shown in \autoref{fig:PDF}.

If we observe the bounds of these three candidates without calculating exact probabilities, we can estimate that \( c_2 \) is less likely to achieve the highest score compared to the others. While unknown questions could potentially impact the outcome, common unknown questions between candidates will affect all candidates similarly and are not game-changers. Therefore, when we exclude their influence, \( P(c_2 = c^*) \) becomes even lower. This is reasonable, as unknown questions cannot help \( c_2 \) exceed its score relative to the others.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/PDF.png}
    \caption{Probability Distribution of the winner candidate}
    \label{fig:PDF}
\end{figure}

\end{example}


\subsection{Determining the Next Question}
\label{uncertainty}

%Define entropy

% design an example of already asked questions, compute entropy, select two question, compare their effect on entropy, why one is better than another

% hence, we propose algorithm to find a question which most likey reduces entropy maximally compared to others

In \autoref{winning_probability}, we demonstrated how to compute the winning probability distribution over candidates. If the winner candidate $c^*$ is known, the uncertainty in finding the query answer is $0$, and we do not need to ask any further questions. Otherwise, we need to keep asking questions from expert to reduce the uncertainty of finding $c^*$. Hence, the key point is to find out what is the next best question to ask expert to reduce uncertainty as much as possible. 

Therefore, we use entropy to define define the uncertainty of $c^*$ as follows:

\[
H(c^*) = - \sum_{i=1}^{n} p(c_i = c^*) \log p(c_i = c^*)
\]

Where $c_i$ is the $i$-th one among all n candidates.  

Hence, we need to select a question from unknown information which potentially reduces the entropy as much as possible. However, since the response to such questions is not known without asking them, we cannot claim for sure how they are going to change the candidates' bounds, and consequently, we do not know for sure how the probability distribution function changes by such a question without asking it. Therefore, it cannot be guaranteed how much the entropy is reduced by a question before asking it. 

Although we cannot predict how exactly a question changes the entropy, since each call to an expert is costly, it is important to find the winner candidate by as minimum number of questions as possible. We have proposed an algorithm called "EntrRed", which at a given point in time, selects a question to ask next which is most likely to reduce the entropy maximally. 

\textbf{EntrRed:} In this algorithm, we first choose the candidate that has the highest probability to be the winner given the bounds. Since such candidate has the highest probability of being the winner, asking a question about this specific candidate is most likely to find the winner candidate and reduce entropy maximally. After picking such candidate, we evaluate each question among the unknown questions contributing to that candidate's score by computing a score for each, and then, we choose the question with the highest such score. This is how the score of a question is computed in this approach:

Given an unknown question $Q$, let $C_Q$ represent the subset of all candidates whose scores are influenced by $Q$, and $C'_Q$ be other candidates. The score assigned to the question $Q$ is the sum of absolute difference between winning probability of candidates in $C_Q$ and winning probability of candidates in $C'_Q$. Intuitively, if the absolute differences in the winning probability of candidates between $C_Q$ and $C'_Q$ is high, it means that asking this question can potentially prune out a lot of candidates from $C_Q$ and $C'_Q$ which previously had significant lower winning probabilities.

Algorithm 2 represents the pseudocode for the question evaluation function (QEF) that was described to evaluate a question, and assign a score to it. Algorithm 3 demonstrates the pseudocode for the EntrRed algorithm which uses QEF defined in Algorithm 2. 

\begin{algorithm}
\caption{Question Evaluation Function}
\begin{algorithmic}[1]
    \Function{evaluate\_question}{Q, $C_Q$}
        \State Initialize $score(Q) \gets 0$
        \For{each candidate $c \in C_Q$}
            \State Initialize $prob\_diff\_sum(c) \gets 0$
            \For{each candidate $c' \notin C_Q$}
                \State $prob\_diff(c,c') \gets \left| p(c) - p(c') \right|$
                \State $prob\_diff\_sum(c) \gets prob\_diff\_sum(c) + prob\_diff(c,c')$
            \EndFor
            \State $score(Q) \gets score(Q) + prob\_diff\_sum(c)$
        \EndFor
        \State \Return $score(Q)$
    \EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{EntrRed Algorithm}
\begin{algorithmic}[1]
    \State \textbf{Input:} Set of unknown questions $\mathcal{Q_U}$, Probability Density Function (PDF) for candidates
    \State \textbf{Output:} A single question $Q^*$ to be asked next
    \State Initialize $Q^* \gets \text{null}$
    \State Initialize $max\_prob \gets -\infty$
    \State Initialize $c^* \gets \text{null}$  \Comment{Candidate with highest probability}
    
    \For{each candidate $c$}
        \State $prob(c) \gets \text{PDF}(c)$ \Comment{Obtain probability of candidate $c$}
        \If{$prob(c) > max\_prob$}
            \State $max\_prob \gets prob(c)$
            \State $c^* \gets c$  \Comment{Update best candidate}
        \EndIf
    \EndFor

    \State Let $Q_{c^*}$ be the set of questions contributing to the score of $c^*$
    \State Initialize $max\_score \gets -\infty$
    \For{each question $Q \in Q_{c^*}$}
        \State $score(Q) \gets \text{Evaluate\_Question}(Q, C_Q)$ \Comment{$C_Q$: candidates influenced by $Q$}
        \If{$score(Q) > max\_score$}
            \State $max\_score \gets score(Q)$
            \State $Q^* \gets Q$  \Comment{Update best question}
        \EndIf
    \EndFor
    
    \State \textbf{return} $Q^*$
\end{algorithmic}
\end{algorithm}



\begin{comment}
    
\textbf{Max Overlap Algorithm:} In this algorithm, we compute a score for each question, and choose the one candidate with the highest overall score. This is how the score of a question is computed in this approach:

Given an unknown question $Q$, let $C_Q$ represent the subset of all candidates whose scores are influenced by $Q$. The score assigned to the question $Q$ is the sum of overlapping areas between the score bounds of candidates in $C_Q$ and other candidates. Intuitively, the overlap between the score bounds of two candidates indicates uncertainty in determining which one is better than the other. If a question frequently appears among candidates with high overlaps, asking that question can be particularly effective in reducing uncertainty and separating the score bounds of overlapping candidates as much as possible. Algorithm 2 represents the pseudocode for the question evaluation function (QEF) that we use to evaluate a question, and assign a score to it. Algorithm 3 demonstrates the pseudocode for the Max Overlap algorithm which works based on the function defined in Algorithm 2. 

\textbf{Running Time Analysis. }The algorithm iterates over all unknown questions ($O(|Q_U|)$). For each unknown question, we iterate over all candidates influenced by it and compute their overlaps with every other candidate $(O(n^2))$. Therefore, the running time of this algorithm is asymptotically $O(|Q_U| \cdot n^2)$.




\begin{algorithm}
\caption{Question Evaluation Function}
\begin{algorithmic}[1]
    \Function{evaluate\_question}{Q, $C_Q$}
        \State Initialize $score(Q) \gets 0$
        \For{each candidate $c \in C_Q$}
            \State Initialize $overlap\_sum(c) \gets 0$
            \For{each candidate $c' \notin C_Q$}
                \State $overlap(c,c') \gets \max(0,\min(UB_c,UB_{c'}) - \max(LB_c,LB_{c'}))$
                \State $overlap\_sum(c) \gets overlap\_sum(c) + overlap(c, c')$
            \EndFor
            \State $score(Q) \gets score(Q) + overlap\_sum(c)$
        \EndFor
        \State \Return $score(Q)$
    \EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Max Overlap Algorithm}
\begin{algorithmic}[1]
    \State \textbf{Input:} Set of unknown questions $\mathcal{Q_U}$
    \State \textbf{Output:} A single question $Q^*$ with the maximum score
    \State Initialize $Q^* \gets \text{null}$
    \State Initialize $max\_score \gets -\infty$
    \For{each question $Q \in \mathcal{Q_U}$}
        \State Let $C_Q$ be the set of candidates affected by $Q$
        \State $current\_score \gets \text{Evaluate\_Question}(Q, C_Q)$
        \If{$current\_score > max\_score$}
            \State $max\_score \gets current\_score$
            \State $Q^* \gets Q$
        \EndIf
    \EndFor
    \State \textbf{return} $Q^*$
\end{algorithmic}
\end{algorithm}

\textbf{Max Probability Algorithm:} In this heuristic, we first choose the candidate that has the highest probability to be the winner given the bounds. Then, among the questions contributing to that candidate's score, we choose one that has the highest share of participation in the overlapping area of the candidates' bounds. Algorithm 4 represents the pseudocode of this heuristic to find the next best question.

\textbf{Running Time Analysis. } In this algorithm, we first select the candidate with the highest probability of being the winner ($O(n)$). Then, we iterate over questions participating in that candidate's score, and for any candidate that is influenced by this question, we sum up its overlap with other candidates ($O(n^2)$). Hence, the running time for this algorithm is asymptotically $O(n + |Q_U| \cdot n^2)$ which can be simplified as $O(|Q_U| \cdot n^2)$.



\begin{algorithm}
\caption{Max Probability Algorithm}
\begin{algorithmic}[1]
    \State \textbf{Input:} Set of unknown questions $\mathcal{Q_U}$, Probability Density Function (PDF) for candidates
    \State \textbf{Output:} A single question $Q^*$
    \State Initialize $Q^* \gets \text{null}$
    \State Initialize $max\_prob \gets -\infty$
    \State Initialize $c^* \gets \text{null}$  \Comment{Candidate with highest probability}
    
    \For{each candidate $c$}
        \State $prob(c) \gets \text{PDF}(c)$ \Comment{Obtain probability of candidate $c$}
        \If{$prob(c) > max\_prob$}
            \State $max\_prob \gets prob(c)$
            \State $c^* \gets c$  \Comment{Update best candidate}
        \EndIf
    \EndFor

    \State Let $Q_{c^*}$ be the set of questions contributing to the score of $c^*$
    \State Initialize $max\_score \gets -\infty$
    \For{each question $Q \in Q_{c^*}$}
        \State $score(Q) \gets \text{evaluate\_question}(Q)$
        \If{$score(Q) > max\_score$}
            \State $max\_score \gets score(Q)$
            \State $Q^* \gets Q$  \Comment{Update best question}
        \EndIf
    \EndFor
    
    \State \textbf{return} $Q^*$
\end{algorithmic}
\end{algorithm}

\end{comment}

\begin{example}
    Following Example 3.6, we can compute the entropy of \( c^* \) given the probabilities for each candidate obtained by the PDF as shown in \autoref{fig:PDF}. Hence, we have:

    \[
    H(c^*) = - \sum_{i=1}^{3} p(c_i) \log p(c_i)
    \]

    we can expand the formula and compute the entropy approximately as follows:

    \[
    H(c^*) = - \left( 0.75 \log(0.75) + 0.01 \log(0.01) + 0.24 \log(0.24) \right)
    \]
    \[
    H(c^*) \approx \text{0.604}
    \]
\end{example}

As we ask more questions, we expect the entropy to decrease. Finally, when the winner candidate is obtained, the entropy goes down to zero. 

Now, we need to select the next question to ask the expert based on the EntrRed algorithm that we described. Hence, we first need to select a candidate which we are going to choose one of the unknown questions that contribute to the score of that. As discussed earlier, such a candidate is the one with the highest probability of being the winner at the point in time, which is $c_1$. Among questions influencing the score of $c_1$, two of them are unknown which are $R(HNY)$ and $D(MLN, HYN)$. Hence, we need to compute the associated score of these questions using the Question Evaluation Function (QEF) and choose the one with higher score. Let $C_Q$ represent the set of candidates that Q affects their score. Then, we have
\begin{itemize}
        \item $Q1$ = R(HNY, q): We need to compute the sum of winning probability difference between candidates from $C_{Q1}$ with any other candidates. Since $C_{Q1} = \{c_1, c_2, c_3\}$, there will be no remaining other candidates for computing overlap with these 3. Hence:
        \begin{align*}
            QEF(Q1) = 0
        \end{align*}
        \item $Q2$ = D(MLN, HYN): Since $C_{Q2} = {c_1}$, we need to compute: 

        \begin{align*}
            QEF(Q2) = |p(c_1) - p(c_2)| + |p(c_1) - p(c_3)|
        \end{align*}
        
        Hence, we have:
        \begin{align*}
            QEF(Q2) = 0.74 + 0.51 = 1.25
        \end{align*}
    \end{itemize}
    Since $QEF(Q2) > QEF(Q1)$, we choose $Q2 = D(MLN, HYN)$ as the next question. 

\begin{comment}
    
\begin{itemize}
    \item \textbf{Max Probability Algorithm}: we first need to select a candidate which we are going to choose one of the unknown questions that contribute to the score of that. As discussed earlier, such a candidate is the one with the highest probability of being the winner at the point in time, which is $c_1$. Among questions influencing the score of $c_1$, two of them are unknown which are $R(HNY)$ and $D(MLN, HYN)$. Hence, we need to compute the associated score of these questions using the Question Evaluation Function (QEF) and choose the one with higher score. Let $C_Q$ represent the set of candidates that Q affects their score. Then, we have
    \begin{itemize}
        \item $Q1$ = R(HNY, q): We need to compute the sum of overlap between the pairwise bounds of candidates from $C_Q1$ with any other candidates. Since $C_Q1 = \{c_1, c_2, c_3\}$, there will be no remaining other candidates for computing overlap with these 3. Hence:
        \begin{align*}
            QEF(Q1) = 0
        \end{align*}
        \item $Q2$ = D(MLN, HYN): Since $C_Q2 = {c_1}$, we need to sum the bounds overlap of $c_1$ and $c_2$ with $c_1$ and $c_3$. Hence, we have:
        \begin{align*}
            QEF(Q2) = 1.5 + 1 = 2.5
        \end{align*}
    \end{itemize}
    Therefore, since $QEF(Q2) > QEF(Q1)$, we choose $Q2 = D(MLN, HYN)$ as the next question. 
    
    \item \textbf{Max Overlap algorithm}: In this approach, we need to consider all the unknown questions, compute their QEF, and choose the one with maximum value. Let $C_Q$ represent the set of candidates that Q affects their score. Given our running example, since we have assumed the only candidates are $\{c_1, c_2, c_3\}$, the questions that affect the score of either of these candidates are as follows: 
    \begin{itemize}
        \item Q1 = R(HNY, q) = 0 (as computed earlier)
        
        \item Q2 = D(MLN, HYN) = 0 (as computed earlier)
        
        \item Q3 = D(MLN, SHN): Since $C_Q3 = {c_2}$, we need to sum the bounds overlap of $c_2$ and $c_1$ with $c_2$ and $c_3$. We will have:
        \begin{align*}
            QEF(Q3) = 1.5 + 1 = 2.5
        \end{align*}
        
        \item Q4 = Since $C_Q4 = {c_3}$, we need to sum the bounds overlap of $c_3$ and $c_1$ with $c_3$ and $c_2$. Therefore:
        \begin{align*}
            QEF(Q4) = 1.5 + 1.5 = 3.0
        \end{align*}
    \end{itemize}
    Hence, since $QEF(Q4)$ has the highest value compared to others, we choose $Q4 = D(MLN, WLD)$ as the next question. 
\end{itemize}

\end{comment}


\subsection{Response Processing}
\label{Response_Processing}
After we select the next question to ask the expert(s), we need to process the received response into our desired form. Depending on if we are using a single or multiple experts, and if the expert response is a discrete value or a range, we have 4 different cases as mentioned in :

\begin{enumerate}
    \item \textbf{Single Expert, Single Response}
    \item \textbf{Single Expert, Range Response}
    \item \textbf{Multiple Experts, Range Response}
    \item \textbf{Multiple Experts, Range Response}
\end{enumerate}

In \autoref{sec:section2.3} we formally defined the overall approach showing the process of mapping the responses from either of the above cases to our desired format. Algorithm 4 shows our generalized algorithm to process the experts' responses which covers all the above cases. 

\begin{algorithm}
\caption{Generalized Response Processing Algorithm}
\begin{algorithmic}[1]
\State \textbf{Input:} Set of experts' responses $R$, where each response $R_i$ is a range $(R_{i,1}, R_{i,2})$. If $R_i$ is a single response, set $R_i = (R_i, R_i)$.
\State \textbf{Output:} Probability density function $f_{\mathcal{S}}(r)$ over the set of desired responses $\mathcal{S}$.

\State Initialize $\mathcal{S}^* \gets []$ \Comment{List to store mapped desired responses}
\For{each response $R_i = (R_{i,1}, R_{i,2})$ in $R$}
    \State Initialize $\mathcal{S}_i^* \gets []$ \Comment{Subset of $\mathcal{S}$ for current response range}
    \For{each $r \in \mathcal{S}$}
        \If{$R_{i,1} \leq r \leq R_{i,2}$}
            \State Append $r$ to $\mathcal{S}_i^*$
        \EndIf
    \EndFor
    \For{each $r_j \in \mathcal{S}_i^*$}
        \State Append $r_j$ to $\mathcal{S}^*$
    \EndFor
\EndFor

\State Calculate total number of elements in $\mathcal{S}^*$, denoted as $n^*$
\State Initialize $f_{\mathcal{S}}(r) \gets 0$ for each $r \in \mathcal{S}$

\For{each $r \in \mathcal{S}^*$}
    \State $f_{\mathcal{S}}(r) \gets f_{\mathcal{S}}(r) + \frac{1}{n^*}$ \Comment{Update probability density based on frequency}
\EndFor

\State \textbf{Return} $f_{\mathcal{S}}(r)$
\end{algorithmic}
\end{algorithm}

\begin{example}
    Following the running example, let's assume that we would like to use the max probability algorithm to select the next question. In this case, as reasoned earlier in Example 3.7, the next selected question will be $Q = D(MLN, HYN)$. 
    We need to leverage Algorithm 5 to output a probability density function over the set of desired responses so that it would be further used to update the bounds accordingly. 
    
    Let's assume that we have 3 experts denoted as $E = \{e_1, e_2, e_3\}$ which all return ranges rather than single discrete values (Case 4). Following our initial assumption in the running example, the set of desired responses is $S = {0.0, 0.5, 1.0}$. Imagine that the experts' responses are as follows:

\[
\begin{aligned}
    \text{Response}(e_1) &= (0.0, 0.2), \\
    \text{Response}(e_2) &= (0.0, 0.3), \\
    \text{Response}(e_3) &= (0.5, 1.0)
\end{aligned}
\]

Each response is then mapped to a subset of desired responses as followed:
\[
\begin{aligned}
    \text{Mapped(Response}(e_1)) &= \{0.0\}, \\
    \text{Mapped(Response}(e_2)) &= \{0.0\}, \\
    \text{Mapped(Response}(e_3)) &= \{0.5, 1.0\}
\end{aligned}
\]

Therefore, by aggregating the obtained mapped responses, we can get the PDF of the experts responses, denoted as PDF(E), as shown in \autoref{fig:Response_PDF}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/Response_PDF.png}
    \caption{Overall Probability Density of the Experts' Responses}
    \label{fig:Response_PDF}
\end{figure}

This PDF is then used to update the bounds. In this case, since the PDF is nonuniform, the updated bounds will be nonuniform as well. In more detail, in this case, if $(LB, UB)_c = (\alpha, \beta)$, the potential score values within this range may no longer be equally probable, and can have different probabilities associated with them. 

\end{example}

==> datamodel_old.tex <==
\section{Data Model, Problem Definition, Proposed Framework}
We describe our data model, specify our problem definition, and present our propose framework.

\subsection{Data Model}
\textbf{Input Query:} A user writes a query $q$ with an input parameter $k$, with the goal of obtaining the top-$k$ set of entities to $q$.

\begin{example}
    The input query can be $q$ = "Affordable hotels in Manhattan" and $k = 3$. It means the goal is to find the top-3 hotels with respect to q.  
\end{example}

\textbf{Database.} The query comes to a database $D$ containing data of different modalities, such as, pictures, text, audio, etc. Item $i$ represents a physical entity $e$ (such as a hotel). There may be multiple items associated with an entity. Let $n$ represent the total number of unique entities.

The toy example \autoref{fig:motivating_scenario} represents the underlying data with $5$ entities or hotels. Each entity has two associated items with it. For instance, the  hotel "HNY", has \{ i1, i3 \} associated with it, an audio and an image file respectively.

\textbf{Scoring function and characteristics.} A user provides a set based scoring function $\mathcal{F}$ that admits a query  $q$ and an integer $k$, and scores any subset $s \subseteq n$ entities, such that $|s|=k$, i.e., $\mathcal{F}(s,q) \rightarrow R$. 

A scoring function needs to satisfy two conditions: (a) it is set based - meaning it computes the score of a set of size $k$ overall and do not provide the individual order of the entities in the set, (b) It is decomposable into a set of constructs, each of these constructs could be sent to an oracle to obtain its predicted value.

\begin{comment}
    \begin{example}
Assume that the scoring function used to evaluate sets is defined as:

\[
\mathcal{F}_{\text{rel+div}}(c, q) = F_{\text{relevance}}(c, q) + F_{\text{diversity}}(c)
\]

Where $F_{\text{relevance}}(c, q)$ is the sum of relevance between query and each entity in that candidate. In other words:

\[
F_{\text{relevance}}(c, q) = \sum_{\text{e} \in c} \text{R}(\text{e}, q)
\]

Similarly, $F_{\text{diversity}}(c)$ is defined as the sum of diversity between any two entities in c:

\[
F_{\text{diversity}}(c) = \sum_{\text{(e1, e2)} \in c}\text{D(e1, e2)}
\]  

Hence, $\mathcal{F}_{\text{rel+div}}(c, q)$ can be used to generate a score for any set of $k$ entities.
\end{example}
\end{comment}





%Now, we can expand the summations and write the overall score formula for any candidate. For instance:

%\[
%\begin{aligned}
%\mathcal{F}(c, q) = & \, F_{\text{relevance}}(c, q) + F_{\text{diversity}}(c) \\
%= & \, R(\text{HNY}) + R(\text{MLN}) + R(\text{HYN}) \\
%  & \, + D(\text{HNY}, \text{MLN}) + D(\text{HNY}, \text{HYN}) + D(\text{MLN}, \text{HYN})
%\end{aligned}
%\]

%similarly, we can expand the formula for computing the score of any other top-3 candidates. Initially, all the candidates are equally probable to be the top-3 set. As we ask the LLM any \( q \in Q \), we gain information that changes the likelihood of each candidate being better than another.

\begin{comment}
    \textbf{Components of a Scoring Function.} Given a scoring function $\mathcal{F}$, the set of components of $\mathcal{F}$ can be denoted by:
\[
\mathcal{S} = \{\mathcal{F}_1, \mathcal{F}_2, \ldots, \mathcal{F}_m\}
\]

where $\mathcal{F}_{\ell}$ denotes the $\ell$-th component. Each component $\mathcal{F}_{\ell}$ may involve individual entities, pairs of entities, or more complex combinations, depending on the nature of the component. Given the required number of entities as input to a component, the score for that set of entities with respect to the component can be computed.
\end{comment}

Imagine a user defined scoring function with the purpose to compute the top-$k$ set that maximizes the sum of relevance and diversity $\mathcal{F}(s, q)= \Sigma_{e \in s} Rel(q,e)+ \Sigma_{e_i,e_j \in s} Div(e_i,e_j)$. The scoring function identifies the top-$k$ set and not the respective order of the entities in the set, and its two constructs can be written as, $Rel(q, e)$ or $Rel(e_i, e_j)$.

\textbf{Top-$k$ set.} Given  a query  $q$ and an integer $k$, a set of entities $E$, and a set based scoring function $\mathcal{F}$, $s_q$ is a top-$k$ set, if $s_q \subseteq E$, $|s_q|=k$, and 
$s_q = argmax_{s \subseteq E: |s|=k} \mathcal{F}(s, q)$.

Given the running example, the following set of 3 hotels denoted as 
 $c_1 = \{ HNY, MLN, HYN \}$ could be the potential set of top-$3$ hotels. However, certainly determining the top-k set requires more insights regarding the unknown values in \autoref{tab:ny_hotels_relevance} and \autoref{tab:ny_hotels_diversity}.
   

\textbf{Oracle calls/Questions.} A question $\mathcal{Q}$ and a user defined scoring function $\mathcal{F}$ (or a call to a DNN, a human expert, or an LLM) is a triple of one of the following two forms: 
\begin{itemize}
    \item $\mathcal{Q}_1$, which is a question of the form $\mathcal{Q}(e_i, q, F_{\ell})$.
    \item $\mathcal{Q}_2$, which is a question of the form $\mathcal{Q}(e_i, e_j, F_{\ell})$.
\end{itemize}
   where $e_i,e_j$ are the $i$-th, $j$-th entities, $q$ is the query, and $F_{\ell}$ is the $\ell$-th component of the scoring function. Depending on the nature of the scoring function, some constructs involve returning a score between a query and one of the two items, e.g., to compute relevance, which requires questions of the form $Q_1$. Some other construct may admit two entities, to compute diversity, which requires questions of the form $Q_2$.

Considering our running example (example query and scoring function), one can propose different questions about the hotels mentioned in \autoref{tab:ny_hotels_relevance}. For instance, $\mathcal{Q}(HNY, q, relevance)$ asks for the relevance between the hotel HNY and the query q, while $\mathcal{Q}(WLD, SHN, diversity)$ represents a question about the diversity between hotels "WLD" and "SHN".

   
% NOTE; figure 1 change sec column to hotel names
\textbf{Response from oracle.} Given a question \( \mathcal{Q} \), and a pre-specified range of values \([MIN, MAX]\) which the oracle is instructed to respond within, the oracle response \( \mathcal{R} \) is defined to have one of the following two forms:

\begin{itemize}
    \item \( \mathcal{R}_1 = r \in [MIN, MAX] \), where \( r \) is a discrete value within the specified range \([MIN, MAX]\).
    
    \item \( \mathcal{R}_2 = (l, u) \), where \( MIN \leq l < u \leq MAX \) represents a continuous range of values that the oracle can provide as a response.
\end{itemize}

Our framework supports all of these possibilities.


Using the running example, the last column of \autoref{tab:ny_hotels_relevance} and each cell in \autoref{tab:ny_hotels_diversity} represents an oracle response of type $\mathcal{R}_1$. 
    
As an example, for the question $\mathcal{Q}(HYN, q, relevance)$, the oracle returns a discrete value $Relevance(HNY, q) = 0.5$. The [MIN, MAX] response values are assumed to be 0 and 1 respectively. At a given point in time, some responses might be unknown and are denoted by $U$ in these tables.
    
Alternatively, let us assume we wish to have responses of type $\mathcal{R}_2$. In this case, as an instance, for a question like $\mathcal{Q}(WLD, SHN, diversity)$, we could have $Diversity(WLD, SHN) = (0.3, 0.7)$ as the response which is a continuous range rather than a discrete value. 



\subsection{Problem Definition}
Given a scoring function $\mathcal{F}$, we define the set of all possible questions, denoted as \( Q_U \), as the union of decomposable constructs.

Using the running example,  \( Q_U \) contains relevance on each of the $5$ hotels in the data, plus a total of $\binom{5}{2}$ diversity questions on each pairs of hotels. At a given point in time, the response to some of these questions could be known. 

\textbf{Known Information.} Let \( Q_K \) be the set of questions whose  responses are known. Thus, we have:

\[
Q_K = \{ q \in Q_{ALL} \mid \text{response to } q \text{ is known} \}
\]

\textbf{Unknown Information.} Conversely, we can define the unknown information as the set of questions for which the responses have not yet been obtained. This set, denoted as \( Q_{ALL} \), is given by:

\[
Q_U = Q_{ALL} \setminus Q_K
\]

\begin{example}
    Let us assume there are five hotels as mentioned in \autoref{tab:ny_hotels_relevance}, and the scoring function is $\mathcal{F}_{\text{rel+div}}$. The response to each relevance and diversity question has been mapped to a cell in \autoref{tab:ny_hotels_relevance} and \autoref{tab:ny_hotels_diversity}, respectively. Cells marked as $U$ indicate an unknown value for that specific question. Hence, based on these two tables, we have:

\[
Q_K = \left\{
\begin{array}{lll}
R(\text{MLN}, q) & R(\text{WLD}, q) & R(\text{HNY}, q) \\
D(\text{HNY}, \text{MLN}) & D(\text{MLN}, \text{HNY}) & D(\text{SHN}, \text{WLD}) \\
D(\text{HYN}, \text{SHN}) & &
\end{array}
\right.
\]


\[
Q_U = \left\{
\begin{array}{lll}
R(\text{HYN}, q) & R(\text{SHN}, q) & D(\text{HYN}, \text{HNY}) \\
D(\text{HYN}, \text{MLN}) & D(\text{HYN}, \text{WLD}) & D(\text{HNY}, \text{HYN}) \\
D(\text{MLN}, \text{HYN}) & D(\text{SHN}, \text{HYN}) &
\end{array}
\right.
\]

We aim to find out what is the next best question to know which is going to be most useful in finding the query answer. 

\end{example}



\begin{table}[h!]
\centering
\begin{tabular}{|c|l|c|}
\hline
\textbf{Abbreviation} & \textbf{Hotel Name} & \textbf{Relevance} \\ \hline
HNY & Hilton NY      & U \\ \hline
MLN & Marriott LN    & 1.0 \\ \hline
HYN & Hyatt NY       & 1.0 \\ \hline
SHN & Sheraton NY    & 0.0 \\ \hline
WLD & Waldorf NY     & 0.5 \\ \hline
\end{tabular}
\caption{Hotels and their relevance to the query "Affordable hotels in Manhattan"}
\label{tab:ny_hotels_relevance}
\end{table}



\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
       & HNY  & MLN  & HYN  & SHN  & WLD  \\ \hline
HNY    & -   & 1.0  & 0.5    & 0.5  & 0.5  \\ \hline
MLN    & 1.0  & -    & U    & U  & U  \\ \hline
HYN    & 0.5    & U    & -    & U  & 0.5    \\ \hline
SHN    & 0.5  & U  & U  & -    & U  \\ \hline
WLD    & 0.5  & U  & 0.5   & U  & -    \\ \hline
\end{tabular}
\caption{Diversity scores between pairs of hotels. Some values are unknown.}
\label{tab:ny_hotels_diversity}
\end{table}





\textbf{Problem Definition:} Given \( n \) entities, k, an input query \( q \), and a user defined set based scoring function \( \mathcal{F} \), already known information \( Q_K \), identify the next question to be asked to the oracle that has the highest likelihood of identifying the true top-$k$ set.

\begin{example}
\label{example2.3}
    Given the running example, Assume we want to find the top-3 hotels with respect to the query "affordable hotels in Manhattan". Assume that at a given point in time, some information is already known which is shown in \autoref{tab:ny_hotels_relevance} and \autoref{tab:ny_hotels_diversity}. For simplicity, let's imagine the ultimate query answer is going to be chosen among either of the following three sets, meaning that we disregard any other possible sets rather than these:
    
    \[
    c_1 = \{\text{HNY, MLN, HYN}\}, 
\]
\[
    c_2 = \{\text{HNY, MLN, WLD}\},
\]
\[
    c_3 = \{\text{HNY, HYN, SHN}\}
\]

    Hence, we aim to find the next best question to ask which is most useful in finding the query answer, which is the top-k set with the highest score.
    
    Potentially, the next question could be any of the cells marked as U (Unknown) in \autoref{tab:ny_hotels_relevance} or \autoref{tab:ny_hotels_diversity}. For simplicity, let's consider two possible questions to ask, and compare how useful they can be:
    
    \begin{itemize}
        \item \( Q_1 \): \(D(MLN, HYN)\) - the diversity score between MLN and HYN
        \item \( Q_2 \): \(D(HYN, SHN)\) - the diversity score between HYN and SHN
    \end{itemize}

    Before asking any of these two questions, by using the known values have:

\[
\begin{aligned}
    \mathcal{F}(c_1, q) = 
    & R(\text{HNY}) + R(\text{MLN}) + R(\text{HYN}) + D(\text{HNY, MLN}) \\
    & + D(\text{HNY, HYN}) + D(\text{MLN, HYN}) \\
    = & 3.5 + R(\text{HNY}) + D(\text{MLN, HYN}) \\
\end{aligned}
\]

\[
\begin{aligned}
    \mathcal{F}(c_2, q) = 
    & R(\text{HNY}) + R(\text{MLN}) + R(\text{WLD}) + D(\text{HNY, MLN}) \\
    & + D(\text{HNY, WLD}) + D(\text{MLN, WLD}) \\
    = & 3.0 + R(\text{HNY}) + D(\text{MLN, WLD}) 
\end{aligned}
\]


\[
\begin{aligned}
    \mathcal{F}(c_3, q) = 
    & R(\text{HNY}) + R(\text{HYN}) + R(\text{SHN}) + D(\text{HNY, HYN}) \\
    & + D(\text{HNY, SHN}) + D(\text{HYN, SHN}) \\
    = & 2.0 + R(\text{HNY}) + D(\text{HYN, SHN}) 
\end{aligned}
\]



    
    Suppose we choose to ask \( Q_1 \), revealing that \(D(MLN, HYN) = 1.0 \). Knowing this additional information, we update the overall scores of \( c_1 \) as follows:
    
\[
\begin{aligned}
    \mathcal{F}(c_1, q) = 
     & 4.5 + R(\text{HNY}) \\
\end{aligned}
\]

    Since all the known/unknown values are within a pre-specified range (In this example: (0, 1)), regardless of the values of remaining unknown variables in $\mathcal{F}(c_2, q)$, $\mathcal{F}(c_1, q)$, and $\mathcal{F}(c_1, q)$, we will have:

    \[
\begin{aligned}
    \mathcal{F}(c_1, q) \geq \mathcal{F}(c_2, q) \quad \text{AND} \quad
    \mathcal{F}(c_1, q) \geq \mathcal{F}(c_3, q)
\end{aligned}
\]

    Hence, in this case, we can conclude that $c_1$ is the query answer. By asking \(D(MLN, HYN)\) from expert, we could potentially get some other answer rather than $1.0$ as well. However, in this example, if \(D(MLN, HYN) \geq 0.5 \), we could still come up with the same conclusion as we did. Therefore, asking \(D(MLN, HYN)\) can likely result in finding the top-3 set.  

    On the other hand, Suppose we choose to ask \( Q_2 \), resulting in \(D(MLN, HYN) = 1.0 \). Knowing this additional information, we update the overall scores of \( c_3 \) as follows:
    
    \[
    \begin{aligned}
        \mathcal{F}(c_3, q) = 
         & 3.0 + R(\text{HNY}) \\
    \end{aligned}
    \]

    In this case, the top-3 set is not clear yet. In more detail, based on different possible values of $D(MLN, HYN)$ and $D(HYN, SHN)$ corresponding to $c_1$ and $c_2$ respectively, any of them could have higher final score than the other. Hence, asking $Q_2$ will determine the top-k set. 

    Generally, At a given point in time, there might be more than one question that could likely determine the top-k set. On the other hand, there might be no question that could determine the top-k set at a specific time, but choosing one question over another might result in fewer number of required questions to ask in the future for finding out the top-k set. 
        
    Hence, it is crucial at each point in time to ask the question that is most likely going to reduce the uncertainty in finding the top-k set and guide us toward identifying the query answer.
\end{example}


%In Section ~\ref{sec:section2.3}, we introduce each component in our proposed framework to solve this problem.





==> extra.tex <==
\begin{definition}
    \textbf{Response Processing. }Let $\mathcal{Q}$ be a given question, and let $R = \{R_1, R_2, \ldots, R_n\}$ represent the set of responses from $n$ different experts. Suppose there is a set of desired possible responses $\mathcal{S} = \{r_1, r_2, \ldots, r_l\}$, where each $r_i$ represents a potential valid answer to be evaluated.
   \end{definition}

Response processing can be defined as a mapping from the set of experts' answers $R$ to a probability density function (PDF) over the set of desired responses $\mathcal{S}$. This process generates a PDF $f_{\mathcal{S}}(r)$, representing the probability density over $\mathcal{S}$, indicating the likelihood of each desired response $r_i \in \mathcal{S}$, given the set of experts' answers $R$. 

Hence, we can formulate this task as follows:

\[
\text{Response Processing}: R \mapsto f_{\mathcal{S}}(r), \quad r \in \mathcal{S}.
\]

The definition can be further elaborated based on the number of experts (single vs. multiple) and the nature of responses (single  vs. a range of responses). This leads to four possible cases:
\textbf{Single Expert, Single Response:} Let a single expert provide one single response $R_1$. The  processing maps this response to a corresponding desired response $r^* \in \mathcal{S}$, where this mapping can be written as:
\begin{align*}
    R_1 \mapsto r^*, \quad r^* \in \mathcal{S}
\end{align*}


The probability density function $f_{\mathcal{S}}(r)$ over the set of desired responses $\mathcal{S}$ is then given by:

\begin{align*}
f_{\mathcal{S}}(r) =
\begin{cases}
1 & \text{if } r = r^* \\
0 & \text{if } r \neq r^*
\end{cases}
\end{align*}


This mapping assigns the probability 1 to the specific response $r^*$ that is derived from the expert's response $R_1$, and 0 to all other responses in $\mathcal{S}$.

\textbf{Single Expert, Range of Responses:} Let a single expert provide a range of responses denoted by $(R_{1,i}, R_{1,j})$, where $R_{1,i}$ and $R_{1,j}$ represent the lower and upper bounds of the response range, respectively. The response processing maps this range to a corresponding subset of desired responses $\mathcal{S}^* \subseteq \mathcal{S}$. In other words:

\begin{align*}
(R_{1,i}, R_{1,j}) & \mapsto \mathcal{S}^* = \{r_1, r_2, \ldots, r_k\}, \\
& \quad \mathcal{S}^* \subseteq \mathcal{S}, \quad k \geq 1.
\end{align*}


The probability density function $f_{\mathcal{S}}(r)$ over the set of desired responses $\mathcal{S}$ is then defined as:

\begin{align*}
f_{\mathcal{S}}(r) = 
\begin{cases}
\frac{1}{k}, & \text{if } r \in \mathcal{S}^*, \\
0, & \text{if } r \notin \mathcal{S}^*.
\end{cases}
\end{align*}


This mapping assigns an equal probability of $\frac{1}{k}$ to each response in the subset $\mathcal{S}^*$, derived from the range $(R_{1,i}, R_{1,j})$, and a probability of 0 to all other responses in $\mathcal{S}$.


{\bf Multiple Experts, Single Response Each:} Let multiple experts provide single responses, denoted by the set $R = \{R_1, R_2, \ldots, R_n\}$, where $n$ is the number of experts. Each expert response $R_i$ is mapped to an element in the set of desired responses $\mathcal{S}$. In other words:

\begin{align*}
R_i \mapsto r_i, \quad & r_i \in \mathcal{S}, \quad i = 1, 2, \ldots, n.
\end{align*}


The list of aggregated mapped responses is denoted as $\mathcal{S}^* = [r_1, r_2, \ldots, r_n]$, where each $r_i$ is derived from $R_i$.

The probability density function $f_{\mathcal{S}}(r)$ over the set of desired responses $\mathcal{S}$ is then defined based on the frequency of each response in the list $\mathcal{S}^*$:

\begin{align*}
f_{\mathcal{S}}(r) &= \frac{\text{count}(r)}{n}, \quad \forall r \in \mathcal{S}.
\end{align*}


where $\text{count}(r)$ denotes the number of times the response $r$ appears in the list $\mathcal{S}^*$. 



\textbf{Multiple Experts, Range of Responses Each:} Let multiple experts provide a range of responses each, denoted by $(R_{i,1}, R_{i,2})$ for the $i$-th expert, where $R_{i,1}$ and $R_{i,2}$ represent the lower and upper bounds of the response range for expert $i$. The set of experts' responses is given by $R = \{(R_{1,1}, R_{1,2}), (R_{2,1}, R_{2,2}), \ldots, (R_{n,1}, R_{n,2})\}$ for $n$ experts.

Each expert's range of responses $(R_{i,1}, R_{i,2})$ is mapped to a subset of desired responses $\mathcal{S}_i^* \subseteq \mathcal{S}$:

\begin{align*}
(R_{i,1}, R_{i,2}) & \mapsto \mathcal{S}_i^* = \{r_{i,1}, r_{i,2}, \ldots, r_{i,k_i}\}, \\
& \quad \mathcal{S}_i^* \subseteq \mathcal{S}, \quad k_i \geq 1.
\end{align*}


The overall mapping results in a list of desired responses denoted as $\mathcal{S}^*$, which is an aggregation of each $\mathcal{S}_i^*$. In other words:

\begin{align*}
\mathcal{S}^* = \left[ r_{1,1}, r_{1,2}, \ldots, r_{1,k_1}, \; 
                     r_{2,1}, r_{2,2}, \ldots, r_{2,k_2}, \; 
                     \ldots, \; 
                     r_{n,1}, r_{n,2}, \ldots, r_{n,k_n} \right]
\end{align*}


The probability density function $f_{\mathcal{S}}(r)$ over the set of desired responses $\mathcal{S}$ is then determined by the frequency of each response $r$ in the list $\mathcal{S}^*$, divided by the total number of elements in $\mathcal{S}^*$, denoted as $n^*$:

\[
f_{\mathcal{S}}(r) = \frac{\text{count}(r)}{n^*}, \quad \forall r \in \mathcal{S}.
\]


where $\text{count}(r)$ denotes the number of times the response $r$ appears in the list $\mathcal{S}^*$. 




Imagine we have two experts ($e_1$ and $e_2$) each of which returns a range of response (case d).
For simplicity, imagine the set of desired responses S is defined as follows:
        \begin{align*}
            S = \{0.0, 0.5, 1.0\}
        \end{align*}

        Given the running example, let's assume we ask  $Q_1 = D(MLN, HYN)$ as the next question, and we get the following responses from the two experts:

        \[
R_{e1} = (0.4, 1.0), \quad R_{e2} = (0.3, 0.6)
\]

Next, we map the above responses to elements of \( \mathcal{S} \) as follows:

\begin{align*}
    e_1: \quad (R_{e1, 1}, R_{e1, 2}) & = (0.4, 1.0) \mapsto \mathcal{S}_1^* = \{0.5, 1.0\} \\
    e_2: \quad (R_{e2, 1}, R_{e2, 2}) & = (0.3, 0.6) \mapsto \mathcal{S}_2^* = \{0.5\}
\end{align*}


Then, we aggregate the two sets together:

\begin{align*}
    \mathcal{S}^* & = [0.5, 1.0, 0.5]
\end{align*}


Then, we can compute the probability density function over the set of desired responses \( \mathcal{S} \) as follows:

\begin{align*}
    f_{\mathcal{S}}(r) & = \frac{\text{count}(r)}{n^*} \\
                       & = \frac{\text{count}(r)}{3}, \quad \forall r \in S = \{0.0, 0.5, 1.0\}
\end{align*}


where \( \text{count}(r) \) denotes the number of times the response \( r \) appears in the list \( \mathcal{S}^* \), and $n^*$ is the total number of elements in $S^*$. Finally, we will have:

\begin{align*}
    f_{\mathcal{S}}(r) =
    \begin{cases}
        \frac{0}{3} & r = 0.0 \\
        \frac{2}{3} & r = 0.5 \\
        \frac{1}{3} & r = 1.0 \\
    \end{cases}
\end{align*}



\autoref{fig:algorithm_framework} illustrates the key components of the computational framework. In \autoref{section3}, we provide a detailed description of our algorithm for each component.
% NOTE: Response preparation - also adds a task 5
% NOTE: Number them
% NOTE: Input box has some inputs
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/Algorithmic_Framework.jpg}
    \caption{The five different components of the probability framework that guide the process of identifying the final answer.}
    \label{fig:algorithm_framework}
\end{figure}


Similarly, we update the bounds for \( c_{5} \), \( c_{6} \), \( c_{8} \), \( c_{9} \), and \( c_{10} \). The new candidate set bounds are as follows:

\[
\text{candidates\_set\_bounds} = \{ 
\begin{aligned}
c_1 &: (0, 6), & c_2 &: (0, 6), \\
c_3 &: (0.5, 5.5), & c_4 &: (0, 6), \\
c_5 &: (0.5, 5.5), & c_6 &: (0.5, 5.5), \\
c_7 &: (0, 6), & c_8 &: (0.5, 5.5), \\
c_9 &: (0.5, 5.5), & c_{10} &: (0.5, 5.5) 
\end{aligned}
\}
\]


This candidates set corresponds to a specific time \( t = 1 \), which only \( R(WLD, q) \) has been asked. When the next question is asked (\( t = 2 \)), the candidates set will be updated again.

Now, at (\( t = 2 \)), let's assume we choose a diversity question like \( D(HNY, MLN) \) to ask. \autoref{tab:ny_hotels_diversity} represents the diversity scores for each pair of hotels. Hence, the expert response is \(1.0\) as \( D(HNY, MLN) = 1.0\) in this table. Now, we need to update candidates including both HNY and MLN, which are \( c_{1} \), \( c_{2} \), and \( c_{3} \). For instance, for \( c_{3} \) we will have:

\begin{align*}
\mathcal{F}(c_3, q) & = R(HNY, q) + R(MLN, q) + 0.5 + D(HNY, MLN) \\
          & \quad + D(HNY, WLD) + D(MLN, WLD) \\
          & = R(HNY, q) + R(MLN, q) + 0.5 + 1.0 \\
          & \quad + D(HNY, WLD) + D(MLN, WLD) \\
          & \implies 1.5 \leq \mathcal{F}(c_3, q) \leq 5.5
\end{align*}

Similarly, we update the bounds for \( c_{1} \) and \( c_{2} \). The new candidates set bounds are as follows:

\[
\text{candidates\_set\_bounds} = \{ 
\begin{aligned}
c_1 &: (1.0, 6), & c_2 &: (1.0, 6), \\
c_3 &: (1.5, 5.5), & c_4 &: (0.0, 6.0), \\
c_5 &: (0.5, 5.5), & c_6 &: (0.5, 5.5), \\
c_7 &: (0.0, 6.0), & c_8 &: (0.5, 5.5), \\
c_9 &: (0.5, 5.5), & c_{10} &: (0.5, 5.5)
\end{aligned}
\}
\]

Finally, let's assume we are at the current point in time, when we have asked all the questions which have known values in \autoref{tab:ny_hotels_relevance} and \autoref{tab:ny_hotels_diversity}, resulting in those two tables. If we update the bounds accordingly based on all the known values, we will have up-to-date bounds as follows:

\[
\text{candidates\_set\_bounds} = \{ 
\begin{aligned}
c_1 &: (3.5, 5.5), & c_2 &: (2.5, 4.5), \\
c_3 &: (3.0, 5.0), & c_4 &: (2.0, 4.0), \\
c_5 &: (3.0, 4.0), & c_6 &: (1.5, 3.5), \\
c_7 &: (2.0, 5.0), & c_8 &: (3.0, 5.0), \\
c_9 &: (1.5, 4.5), & c_{10} &: (2.0, 4.0)
\end{aligned}
\}
\]


==> probabilitymodel_old.tex <==

\subsection{High-Level Taks in Computational Framework}\label{sec:section2.3}
Our proposed framework consists of five essential tasks in the overall top-k selection process:

\begin{enumerate}
    \item \textbf{Task 1: Identifying the Candidates' Set}: 
    %\begin{definition}
    %{\bf Candidate.} A candidate c is a set of $k$-entities that could potentially be produced as the answer to the query.
    %\end{definition}

    %\begin{definition}
     %   {\bf Candidates set.} A set $\mathcal{C}$ containing any possible candidate c which is likely to be the top-k set at a given point in time. 
    %\end{definition}

    Depending on the underlying scoring function and algorithm, the framework identifies one, several, or all candidate top-$k$ sets as answers to the query.
    
    \begin{example}
        Using the running example, two possible candidates could be: 
        \[
        c_1 = \{\text{HNY, MLN, HYN}\}, \quad c_2 = \{\text{MLN, HYN, WLD}\}
        \]
        Hence, we can define the candidates' set C as follows:
        \[
        C = \{c1, c2\}
        \]
        
    \end{example}
    
    \item \textbf{Task 2: Computing bounds of Candidates}: 
         \begin{definition}
     {\bf Lower and upper bounds of a candidate.} Given a scoring function $\mathcal{F}$, and the known information $Q_K$, the lower bound (resp. upper bound) of score of c is the smallest (resp. largest) score that c can have.
    \end{definition}

    \begin{example}
        Considering our running example, let us assume we are interested in finding the bounds for c1:
        \[
        c_1 = \{\text{HNY, MLN, HYN}\}
        \]
        Given $\mathcal{F}_{\text{rel+div}}$ as the scoring function, we can compute the score of c1 as follows:
        
        
        \begin{align*}
            \mathcal{F}(c_1, q) = 
            &R(\text{HNY}) + R(\text{MLN}) + R(\text{HYN}) + D(\text{HNY, MLN}) \\
            &+ D(\text{HNY, HYN}) + D(\text{MLN, HYN})
        \end{align*}

    
        To find the lowest and highest possible scores of $c_1$, we should replace known values from \autoref{tab:ny_hotels_relevance} and \autoref{tab:ny_hotels_diversity} in the above formula and substitute unknown values in the formula with minimum and maximum possible response values which are assumed to be 0 and 1 respectively. Therefore, we can compute the minimum and maximum overall scores of $c_1$:
\[
\mathcal{F}_{\text{min}}(c_1, q) = R(\text{HNY}) + R(\text{MLN}) + 0 + D(\text{HNY, MLN}) + 0 + 0
\]
\[
\mathcal{F}_{\text{min}}(c_1, q) = 0.5 + 1.0 + 0 + 0.5 + 0 + 0 = 2.0
\]

\[
\mathcal{F}_{\text{max}}(c_1, q) = R(\text{HNY}) + R(\text{MLN}) + 1 + D(\text{HNY, MLN}) + 1 + 1
\]
\[
\mathcal{F}_{\text{max}}(c_1, q) = 0.5 + 1.0 + 1 + 0.5 + 1 + 1 = 5.0
\]

Therefore, the lower bound (LB) and upper bound (UB) of \( c_1 \) are:
\begin{align*}
    (\text{LB, UB})_{c_1} &= (2.0, 5.0)
\end{align*}
    
    \end{example}

   
    \item \textbf{Task 3: Probabilistic Model for finding the answer}: 
Given the space of candidates set, query answer is modeled as a discrete random variable $\mathcal{A}$ that takes one candidate $c \in C$, with the probability associated with $c$ to be the answer.
  \begin{definition}
    {\bf Probability of a candidate being the answer.} Given a set $\mathcal{C} = 
    \{c_1, c_2, \ldots, c_m\}$, the probability that $c_i$ is the answer of the query can be formally written as: 
    
    \begin{align*}
    P(c_i = \text{winner}) &= P\left(\bigcap_{c_j \in \mathcal{C}} \mathcal{F}(c_i, q) \geq \mathcal{F}(c_j, q)\right)
\end{align*}

\end{definition}

    \begin{example}
    Let's consider the scenario described in Example \ref{example2.3}, having 3 possible candidates $c_1, c_2$, and $c_3$. Imagine we want to evaluate the chance of $c_1$ being the query answer. For each candidate we have:

    \[
\begin{aligned}
    \mathcal{F}(c_1, q) 
    = & 3.5 + R(\text{HNY}) + D(\text{MLN, HYN}) \\
    \mathcal{F}(c_2, q) 
    = & 3.0 + R(\text{HNY}) + D(\text{MLN, WLD}) \\
    \mathcal{F}(c_3, q) 
    = & 2.0 + R(\text{HNY}) + D(\text{HYN, SHN}) 
\end{aligned}
\]  

Hence, it is trivial that: 

\begin{align*}
    0 < P(c_3 = \text{winner}) < P(c_2 = \text{winner}) < P(c_1 = \text{winner}) < 1
\end{align*}

Following the same scenario as described in Example \ref{example2.3}, if we ask $Q_1 = D(MLN, HYN)$ and get \(D(MLN, HYN) = 1.0 \), regardless of the unknown values, $c_1$ will have higher overall score compared to others. Therefore, in this case, we will have:
\begin{align*}
   P(c_1 = \text{winner}) = 1 \\
   P(c_2 = \text{winner}) = 0 \\
   P(c_3 = \text{winner}) = 0 \\
\end{align*}
It can be observed how asking a question can change the probability of a candidate to be the query answer. Further detail on how to compute the exact winning probability $P(c = \text{winner})$ is mentioned in \autoref{winning_probability}. 

    
    \end{example}
    
    \item \textbf{Task 4: Determining the Next Question}: The next task involves determining the next question to ask. 

 \begin{definition}
     {\bf Uncertainty of $\mathcal{A}$.} {Given $\mathcal{A}$ as the query answer, the uncertainty of finding the top-k set can be formulated as the entropy of $\mathcal{A}$, and it can be written as follows: }
     
    \begin{align*}
    H(\mathcal{A}) &= - \sum_{c \in \mathcal{C}} p_c \log(p_c)
\end{align*}


    Where $p_c$ is the probability of candidate c to be the query answer. 
    \end{definition}

    \begin{example}
        Let's consider the scenario described in Example \ref{example2.3}, having 3 possible candidates $c_1, c_2$, and $c_3$. The uncertainty of the query answer $\mathcal{A}$ can be formulated as:
        \begin{align*}
    H(\mathcal{A}) &= - (p_{c_1} \log(p_{c_1}) + p_{c_2} \log(p_{c_2}) + p_{c_3} \log(p_{c_3}))
    \end{align*}

    Following the same scenario as described in Example \ref{example2.3}, we showed that if we ask $Q_1 = D(MLN, HYN)$ and get \(D(MLN, HYN) = 1.0 \), $c_1$ will be the winner candidate regardless of the unknown values. In other words:
    \begin{align*}
   P(c_1 = \text{winner}) = 1 \\
   P(c_2 = \text{winner}) = 0 \\
   P(c_3 = \text{winner}) = 0 \\
    \end{align*}
    By replacing that in the entropy formula, we will have:
    \begin{align*}
    H(\mathcal{A}) &= - (1 \log(1)) = 0
    \end{align*}

    Hence, after asking \(Q_1\), the query answer is definitively \(c_1\), with no remaining uncertainty. In general, our goal is to identify the next best question that is most likely to maximize the reduction in the entropy of the query answer.
        
    \end{example}
    

   \item \textbf{Task 5: Response Processing}: Instead of relying on a single expert for a question, we could potentially ask it from multiple experts. The goal of a response processing task is to process experts' responses to be used in the bound computation task for updating the bounds.   

\begin{definition}
    \textbf{Response Processing. }Let $\mathcal{Q}$ be a given question, and let $R = \{R_1, R_2, \ldots, R_n\}$ represent the set of responses from $n$ different experts. Suppose there is a set of desired possible responses $\mathcal{S} = \{r_1, r_2, \ldots, r_l\}$, where each $r_i$ represents a potential valid answer to be evaluated.

Response processing can be defined as a mapping from the set of experts' answers $R$ to a probability density function (PDF) over the set of desired responses $\mathcal{S}$. This process generates a PDF $f_{\mathcal{S}}(r)$, representing the probability density over $\mathcal{S}$, indicating the likelihood of each desired response $r_i \in \mathcal{S}$, given the set of experts' answers $R$. 

Hence, we can formulate this task as follows:

\[
\text{Response Processing}: R \mapsto f_{\mathcal{S}}(r), \quad r \in \mathcal{S}.
\]

The definition can be further elaborated based on the number of experts (single vs. multiple) and the nature of responses (single  vs. a range of responses). This leads to four possible cases:

\begin{enumerate}
    \item \textbf{Single Expert, Single Response:} Let a single expert provide one single response $R_1$. The  processing maps this response to a corresponding desired response $r^* \in \mathcal{S}$, where this mapping can be written as:
\begin{align*}
    R_1 \mapsto r^*, \quad r^* \in \mathcal{S}
\end{align*}


The probability density function $f_{\mathcal{S}}(r)$ over the set of desired responses $\mathcal{S}$ is then given by:

\begin{align*}
f_{\mathcal{S}}(r) =
\begin{cases}
1 & \text{if } r = r^* \\
0 & \text{if } r \neq r^*
\end{cases}
\end{align*}


This mapping assigns the probability 1 to the specific response $r^*$ that is derived from the expert's response $R_1$, and 0 to all other responses in $\mathcal{S}$.


    \item \textbf{Single Expert, Range of Responses:} Let a single expert provide a range of responses denoted by $(R_{1,i}, R_{1,j})$, where $R_{1,i}$ and $R_{1,j}$ represent the lower and upper bounds of the response range, respectively. The response processing maps this range to a corresponding subset of desired responses $\mathcal{S}^* \subseteq \mathcal{S}$. In other words:

\begin{align*}
(R_{1,i}, R_{1,j}) & \mapsto \mathcal{S}^* = \{r_1, r_2, \ldots, r_k\}, \\
& \quad \mathcal{S}^* \subseteq \mathcal{S}, \quad k \geq 1.
\end{align*}


The probability density function $f_{\mathcal{S}}(r)$ over the set of desired responses $\mathcal{S}$ is then defined as:

\begin{align*}
f_{\mathcal{S}}(r) = 
\begin{cases}
\frac{1}{k}, & \text{if } r \in \mathcal{S}^*, \\
0, & \text{if } r \notin \mathcal{S}^*.
\end{cases}
\end{align*}


This mapping assigns an equal probability of $\frac{1}{k}$ to each response in the subset $\mathcal{S}^*$, derived from the range $(R_{1,i}, R_{1,j})$, and a probability of 0 to all other responses in $\mathcal{S}$.


    \item \textbf{Multiple Experts, Single Response Each:} Let multiple experts provide single responses, denoted by the set $R = \{R_1, R_2, \ldots, R_n\}$, where $n$ is the number of experts. Each expert response $R_i$ is mapped to an element in the set of desired responses $\mathcal{S}$. In other words:

\begin{align*}
R_i \mapsto r_i, \quad & r_i \in \mathcal{S}, \quad i = 1, 2, \ldots, n.
\end{align*}


The list of aggregated mapped responses is denoted as $\mathcal{S}^* = [r_1, r_2, \ldots, r_n]$, where each $r_i$ is derived from $R_i$.

The probability density function $f_{\mathcal{S}}(r)$ over the set of desired responses $\mathcal{S}$ is then defined based on the frequency of each response in the list $\mathcal{S}^*$:

\begin{align*}
f_{\mathcal{S}}(r) &= \frac{\text{count}(r)}{n}, \quad \forall r \in \mathcal{S}.
\end{align*}


where $\text{count}(r)$ denotes the number of times the response $r$ appears in the list $\mathcal{S}^*$. 



\item \textbf{Multiple Experts, Range of Responses Each:} Let multiple experts provide a range of responses each, denoted by $(R_{i,1}, R_{i,2})$ for the $i$-th expert, where $R_{i,1}$ and $R_{i,2}$ represent the lower and upper bounds of the response range for expert $i$. The set of experts' responses is given by $R = \{(R_{1,1}, R_{1,2}), (R_{2,1}, R_{2,2}), \ldots, (R_{n,1}, R_{n,2})\}$ for $n$ experts.

Each expert's range of responses $(R_{i,1}, R_{i,2})$ is mapped to a subset of desired responses $\mathcal{S}_i^* \subseteq \mathcal{S}$:

\begin{align*}
(R_{i,1}, R_{i,2}) & \mapsto \mathcal{S}_i^* = \{r_{i,1}, r_{i,2}, \ldots, r_{i,k_i}\}, \\
& \quad \mathcal{S}_i^* \subseteq \mathcal{S}, \quad k_i \geq 1.
\end{align*}


The overall mapping results in a list of desired responses denoted as $\mathcal{S}^*$, which is an aggregation of each $\mathcal{S}_i^*$. In other words:

\begin{align*}
\mathcal{S}^* = \left[ r_{1,1}, r_{1,2}, \ldots, r_{1,k_1}, \; 
                     r_{2,1}, r_{2,2}, \ldots, r_{2,k_2}, \; 
                     \ldots, \; 
                     r_{n,1}, r_{n,2}, \ldots, r_{n,k_n} \right]
\end{align*}




The probability density function $f_{\mathcal{S}}(r)$ over the set of desired responses $\mathcal{S}$ is then determined by the frequency of each response $r$ in the list $\mathcal{S}^*$, divided by the total number of elements in $\mathcal{S}^*$, denoted as $n^*$:

\[
f_{\mathcal{S}}(r) = \frac{\text{count}(r)}{n^*}, \quad \forall r \in \mathcal{S}.
\]


where $\text{count}(r)$ denotes the number of times the response $r$ appears in the list $\mathcal{S}^*$. 


\end{enumerate}
\end{definition}


    \begin{example}
        Imagine we have two experts ($e_1$ and $e_2$) each of which returns a range of response (case d).
        
        For simplicity, imagine the set of desired responses S is defined as follows:
        \begin{align*}
            S = \{0.0, 0.5, 1.0\}
        \end{align*}

        Given the running example, let's assume we ask  $Q_1 = D(MLN, HYN)$ as the next question, and we get the following responses from the two experts:

        \[
R_{e1} = (0.4, 1.0), \quad R_{e2} = (0.3, 0.6)
\]

Next, we map the above responses to elements of \( \mathcal{S} \) as follows:

\begin{align*}
    e_1: \quad (R_{e1, 1}, R_{e1, 2}) & = (0.4, 1.0) \mapsto \mathcal{S}_1^* = \{0.5, 1.0\} \\
    e_2: \quad (R_{e2, 1}, R_{e2, 2}) & = (0.3, 0.6) \mapsto \mathcal{S}_2^* = \{0.5\}
\end{align*}


Then, we aggregate the two sets together:

\begin{align*}
    \mathcal{S}^* & = [0.5, 1.0, 0.5]
\end{align*}


Then, we can compute the probability density function over the set of desired responses \( \mathcal{S} \) as follows:

\begin{align*}
    f_{\mathcal{S}}(r) & = \frac{\text{count}(r)}{n^*} \\
                       & = \frac{\text{count}(r)}{3}, \quad \forall r \in S = \{0.0, 0.5, 1.0\}
\end{align*}


where \( \text{count}(r) \) denotes the number of times the response \( r \) appears in the list \( \mathcal{S}^* \), and $n^*$ is the total number of elements in $S^*$. Finally, we will have:

\begin{align*}
    f_{\mathcal{S}}(r) =
    \begin{cases}
        \frac{0}{3} & r = 0.0 \\
        \frac{2}{3} & r = 0.5 \\
        \frac{1}{3} & r = 1.0 \\
    \end{cases}
\end{align*}

    \end{example}
\end{enumerate}

\autoref{fig:algorithm_framework} illustrates the key components of the computational framework. In \autoref{section3}, we provide a detailed description of our algorithm for each component.
% NOTE: Response preparation - also adds a task 5
% NOTE: Number them
% NOTE: Input box has some inputs
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/Algorithmic_Framework.jpg}
    \caption{The five different components of the probability framework that guide the process of identifying the final answer.}
    \label{fig:algorithm_framework}
\end{figure}



==> related_old.tex <==
% \vspace*{-2ex} 
% \vspace*{-1ex} 
\section{Related Work}
\label{sec:related}
Our work is related to approximate query answering, optimizing ML inference, and to combining queries with ML inference. \\

\noindent {\bf Query approximation.}
Approximate query processing is topic that is widely addressed in the database community. The aim is to find approximate answers that are as close as possible to exact answers and that can be found much faster. 
Query approximation techniques~\cite{DBLP:journals/dase/LiL18} can be categorized into (1) online aggregation: select samples online and use them to answer OLAP queries, and (2) offline synopses generation 
 to facilitate OLAP queries. Our work adopts a probabilistic top-k approach~\cite{DBLP:conf/vldb/TheobaldWS04} and is significantly different from these.

\noindent {\bf Optimizing ML inference.}
Several recent approaches were proposed to speed up the application of an ML model. 
Existing approaches follow either an in-database~\cite{DBLP:conf/nsdi/CrankshawWZFGS17} or in-application approach~\cite{DBLP:conf/kdd/AhmedABCCDDEFFG19}. Amazon Aurora is an example of an in-database containerized solution that enables external calls from SQL queries to ML models in SageMaker~\cite{sagemaker_2022}. 
Containerized execution introduces overhead in prediction latency. To mitigate that, Google's BigQuery ML~\cite{bigquery_2022}
and Microsoft's Raven were developed~\cite{DBLP:conf/cidr/KaranasosIPSPPX20}. Compared to Raven, BigQuery ML relies mostly on hard-coded models and targets batch predictions, since it inherits a relatively high startup cost. Raven and its runtime environment ONNX~\cite{DBLP:conf/osdi/ChenMJZYSCWHCGK18} offer the additional ability to make tuple-level inference. 

\noindent{\bf Combining queries and ML inference.}
Our work is closest to combining queries and ML inference since we aim to answer queries over predictions made by those models. This is a research topic that attracted attention recently. We present them here in chronological order. 
Bolukbasi et al.~\cite{DBLP:conf/icml/BolukbasiWDS17} enable  incremental predictions for neural networks.  
 Computation time is reduced by pruning examples that are classified in earlier layers, selected adaptively. 
Kang et al.~\cite{DBLP:journals/pvldb/KangEABZ17} present NOSCOPE, a system for querying videos that can reduce the cost of neural network video analysis by up to three orders of magnitude via inference-optimized model search.
Lu et al.~\cite{DBLP:conf/sigmod/LuCKC18} and Yang et al.~\cite{10.14778/3547305.3547310} use probabilistic predicates to filter data blobs that do not satisfy the query and empirically increase data reduction rates. 
Anderson et al.~\cite{DBLP:conf/icde/AndersonCRW19} use a hierarchical model to reduce the runtime cost of queries over visual content. 
Gao et al.~\cite{DBLP:conf/sigmod/GaoXAY21} introduce a Multi-Level Splitting Sampling to let one "promising" sample path prefix generate multiple "offspring" paths, and direct Monte-Carlo based simulations toward more promising paths. 
Lai et al.~\cite{10.1145/3448016.3452786} studies approximate top-$k$ queries with light-weight proxy models that generate oracle label distribution.
Recent work adopted the use of cheap proxy models, such as image classifiers, to identify  an  approximate  set  of $k$ entities satisfying a query~\cite{DBLP:journals/pvldb/DingAL22,DBLP:journals/pvldb/KangGBHZ20}. 
